Timed Automata Robustness Analysis via Model Checking

Timed automata (TA) have been widely adopted as a suitable formalism to model time-critical systems. Furthermore, contemporary model-checking tools allow the designer to check whether a TA complies with a system specification. However, the exact timing constants are often uncertain during the design phase. Consequently, the designer is often able to build a TA with a correct structure, however, the timing constants need to be tuned to satisfy the specification. Moreover, even if the TA initially satisfies the specification, it can be the case that just a slight perturbation during the implementation causes a violation of the specification. Unfortunately, model-checking tools are usually not able to provide any reasonable guidance on how to fix the model in such situations. In this paper, we propose several concepts and techniques to cope with the above mentioned design phase issues when dealing with reachability and safety specifications.

==> algs/alg_enlarge.tex <==
\DontPrintSemicolon

\ForEach{$c \in (\Psi(\Delta) \cup \Psi(Inv)) \setminus (D \cup I )$}{
	\lIf{$c \in \Psi(\Delta)$ \textbf{and} $\TA_{<D \cup \{c\},I>}$ is sufficient}
	{
		$D \gets D \cup \{c\}$
	}
	\lIf{$c \in \Psi(Inv)$ \textbf{and} $\TA_{<D,I \cup \{c\}>}$ is sufficient}
	{
		$I \gets I \cup \{c\}$
	}
}
\Return $\TA_{<D,I>}$


